Efficient and Flexible Approach to Simulate Low-Dimensional Quantum Lattice Models with Large Local Hilbert Spaces

Quantum lattice models with large local Hilbert spaces emerge across various fields in quantum many-body physics. Problems such as the interplay between fermions and phonons, the BCS-BEC crossover of interacting bosons, or decoherence in quantum simulators have been extensively studied both theoretically and experimentally. In recent years, tensor network methods have become one of the most successful tools to treat lattice systems numerically. Nevertheless, systems with large local Hilbert spaces remain challenging. Here, we introduce a mapping that allows to construct artificial $U(1)$ symmetries for any type of lattice model. Exploiting the generated symmetries, numerical expenses that are related to the local degrees of freedom decrease significantly. This allows for an efficient treatment of systems with large local dimensions. Further exploring this mapping, we reveal an intimate connection between the Schmidt values of the corresponding matrix-product-state representation and the single-site reduced density matrix. Our findings motivate an intuitive physical picture of the truncations occurring in typical algorithms and we give bounds on the numerical complexity in comparison to standard methods that do not exploit such artificial symmetries. We demonstrate this new mapping, provide an implementation recipe for an existing code, and perform example calculations for the Holstein model at half filling. We studied systems with a very large number of lattice sites up to $L=501$ while accounting for $N_{\rm ph}=63$ phonons per site with high precision in the CDW phase.

==> disc_weight_scaling.tex <==
\ifthenelse{\boolean{rebuildCurrentBlock}}%
{%
	\setboolean{removeData}{true}%
}%
{%
	\ifthenelse{\boolean{buildCurrentBlockInline}}%
	{%
		\setboolean{removeData}{true}%
	}{}%
}%
%
\ifthenelse{\boolean{removeData}}%
{%
	\immediate\write18{rm -f \dstdir/scaling.dat}%
}{}%
%
\foreach \L in \Ls%
{%
	\immediate\write18{echo "L: \L" 1>&2}%
	\pgfmathsetmacro{\N}{int(\L/2)}%
%	N=\N%
%
	\def\d{1em04}%
	\immediate\write18{echo "dw E0 convergence discweight" > \datadir/../gs_energies.dat}%%
%	\IfFileExists{\datadir/../gs_fit.dat}{\immediate\write18{rm -f \datadir/../gs_fit.dat}}{}%
%
	\foreach \d in \dws%
	{%
		\ifthenelse{\boolean{rebuildCurrentBlock}}%
		{%
			\IfFileExists{\datadir/log/sym-groundstate-search.output}%
			{%
				\setboolean{rebuildData}{true}%
			}%
			{%
				\setboolean{rebuildData}{false}%		
			}%
		}%
		{%
			\ifthenelse{\boolean{buildCurrentBlockInline}}%
			{%
				\IfFileExists{\datadir/log/sym-groundstate-search.output}%
				{%
					\setboolean{rebuildData}{true}%
				}%
				{%
					\setboolean{rebuildData}{false}%
				}%
			}%
			{%
				\setboolean{rebuildData}{false}%
			}%
		}%
%
		\ifthenelse{\boolean{rebuildData}}%
		{%
			\immediate\write18{rm -f \datadir/../.NoValidResultsDetected.tmp}%
			\immediate\write18%
			{%
%				if [ \string$(grep 'stage \stage c' \datadir/log/sym-groundstate-search.output | wc -l) = 0 ]; then touch  \datadir/../.NoValidResultsDetected.tmp; fi
				if [ \string$(grep '\string^energy' \datadir/log/sym-groundstate-search.output | wc -l) = 0 ]; then touch  \datadir/../.NoValidResultsDetected.tmp; fi
			}%
			\IfFileExists{\datadir/.not_converged}%
			{%
				\immediate\write18{touch  \datadir/../.NoValidResultsDetected.tmp}%
			}{}%
			\IfFileExists{\datadir/../.NoValidResultsDetected.tmp}%
			{%
				\immediate\write18{rm -f \datadir/../.NoValidResultsDetected.tmp}%
			}%
			{%	
%				\immediate\write18%
%				{%
%					echo \d	\
%					\string$(grep -B3 'stage \stage c' \datadir/log/sym-groundstate-search.output | tail -n3 | head -n1 | tr -d , | awk '{print \string$2,\string"\string\t\string",\string$5}') \
%					\string$(grep -B\string$((\L+6)) 'stage \stage c' \datadir/log/sym-groundstate-search.output | tail -n \string$((\L+6)) | sed "s/e-gain /e-gain:/" | awk "{print \string\$12}" | LC_NUMERIC=en_US.UTF-8 sort -g | tail -n1 )	\
%					>>  \datadir/../gs_energies.dat
%				}%
				\immediate\write18%
				{%
					echo \d	\
					\string$(grep '\string^energy' \datadir/log/sym-groundstate-search.output | tail -n1 | tr -d , | awk '{print \string$2,\string"\string\t\string",\string$5}') \
					\string$(grep -B\string$((\L+4)) '\string^energy' \datadir/log/sym-groundstate-search.output | tail -n \string$((\L+4)) | sed "s/e-gain /e-gain:/" | awk "{print \string\$12}" | LC_NUMERIC=en_US.UTF-8 sort -g | tail -n1 )	\
					>>  \datadir/../gs_energies.dat
				}%
			}%
		}{}%
	}%
	%
	\IfFileExists{\datadir/../gs_energies.dat}%
	{
		\immediate\write18%
		{if [ \string$(cat \datadir/../gs_energies.dat | wc -l) = 1 ]; then touch  \datadir/../.NoValidResultsDetected.tmp; fi}%
	}%
	{
		\immediate\write18{touch  \datadir/../.NoValidResultsDetected.tmp}%	
	}%
	\IfFileExists{\datadir/../.NoValidResultsDetected.tmp}%
	{}%
	{%
		\IfFileExists{\datadir/log/sym-groundstate-search.output}%
		{%
			\ifthenelse{\boolean{rebuildCurrentBlock}}%
			{%
				\tikzset{external/remake next=true}%
				\IfFileExists{\datadir/../gs_fit.dat}{\immediate\write18{rm -f \datadir/../gs_fit.dat}}{}%
			}%
			{%
				\ifthenelse{\boolean{buildCurrentBlockInline}}%
				{%
					\tikzset{external/export next=false}%
					\IfFileExists{\datadir/../gs_fit.dat}{\immediate\write18{rm -f \datadir/../gs_fit.dat}}{}%
				}{}%
			}%
			\begin{tikzpicture}%
				\begin{axis}
				[
					opacity	= 0,
					width	=	0.85\textwidth,
					height	=	0.25\textheight,
					xmode	=	log,
					xlabel	=	{\small Discarded weight},
					ylabel	=	{$\nicefrac{E_0}{L}$},
					legend pos	=	north west,
					legend style=
					{
						font=\tiny,
					},
				]
				%	
				\addplot
				[
					color=blue,
					thick,
					only marks,
					mark=x,
					unbounded coords=jump,
					error bars/.cd, 
					y dir=both,
					y explicit,
				] 
					table
					[
						x expr = \thisrowno{3},
						y expr = \thisrowno{1}/(\L),
						y error expr = 2.0*sqrt(\thisrowno{3}/\L), 
					]
					{\datadir/../gs_energies.dat};
				\addlegendentry{DMRG results};
				
				\makeatletter
					\addplot
					[
						no markers, 
						color=blue,
						thick,
					] 
						gnuplot 
						[
							raw gnuplot
						] 
						{
							set fit quiet;
							set fit logfile '/dev/null';
							set print "\datadir/../gs_fit.dat" append;
							set fit errorvariables;
							f(x) = a+abs(b)*x;
							fit f(x) '\datadir/../gs_energies.dat' u ($4):($2) via a,b;
							fit f(x) '\datadir/../gs_energies.dat' u ($4):($2):(2.0*sqrt($4)) yerrors via a,b;
							print \L,\N,a,a_err,b,b_err;
						};
				\makeatother
				
				\IfFileExists{\datadir/../gs_fit.dat}%
				{
					\immediate\write18%
					{if [ \string$(cat \datadir/../gs_fit.dat | wc -l) = 0 ]; then touch  \datadir/../.NoValidFit.tmp; fi}%
				}%
				{
					\immediate\write18{touch  \datadir/../.NoValidResultsDetected.tmp}%	
				}%
				
				\IfFileExists{\datadir/../.NoValidFit.tmp}%
				{
					\immediate\write18{rm -f \datadir/../.NoValidFit.tmp}%	
					\immediate\write18{rm -f \datadir/../.NoValidResultsDetected.tmp}%	
				}
				{
					\pgfplotstableread[header=false]{\datadir/../gs_fit.dat}{\DataUZero}
					\pgfplotstablegetelem{0}{2}\of\DataUZero 
					\pgfmathsetmacro{\Ea}{\pgfplotsretval}
					\pgfplotstablegetelem{0}{3}\of\DataUZero 
					\edef\Eaerr{\pgfplotsretval}
					\pgfplotstablegetelem{0}{4}\of\DataUZero 
					\pgfmathsetmacro{\Eb}{\pgfplotsretval}
					
					\addplot
					[
						domain	=	\xmin:\xmax,
						color=blue,
						dashed,
					]
						{linearFct(\Eb, \Ea)/\L};
					\pgfmathparse{\Ea/\L}
					\edef\E{\pgfmathresult}
					\addlegendentry{fit to $E_0/L=\pgfmathprintnumber[std,precision=4]{\E} \pm \pgfmathprintnumber[sci,precision=2]{\Eaerr}$};
				}
				\end{axis}
			\end{tikzpicture}%
		}{}%
%
		\IfFileExists{\datadir/../gs_fit.dat}%
		{%
			\immediate\write18%
			{%
				grep -v "inf.0" \datadir/../gs_fit.dat | grep -v "NaN" >> \dstdir/scaling.dat
			}%
		}{}%
	}%
}%
\ifthenelse{\boolean{rebuildCurrentBlock}}%
{%
	\IfFileExists{\datadir/log/sym-groundstate-search.output}%
	{%
		\setboolean{rebuildData}{true}%
	}%
	{%
		\setboolean{rebuildData}{false}%		
	}%
}%
{%
	\ifthenelse{\boolean{buildCurrentBlockInline}}%
	{%
		\setboolean{rebuildData}{true}%
	}%
	{%
		\setboolean{rebuildData}{false}%
	}%
}%

\vspace{-0.24\textheight}%


==> the_actual_finite_size_scaling_plot.tex <==
\ifthenelse{\boolean{rebuildCurrentBlock}}%
{%
	\tikzset{external/remake next=true}%
%		\immediate\write18{rm \datadir/gs_fit.dat}%
}%
{%
	\ifthenelse{\boolean{buildCurrentBlockInline}}%
	{%
		\tikzset{external/export next=false}%
%			\immediate\write18{rm \datadir/gs_fit.dat}%
	}{}%
}%

\ifthenelse{\boolean{rebuildData}}%
{%
	\immediate\write18{rm \dstdir/scaling_output.dat}%
}{}%

\tikzset{external/export next=false}%
\tikzsetnextfilename{gs_disc_weight_fit}%
%	
\pgfdeclareplotmark{xocgC}%
{%
	\pgfmathtruncatemacro{\ocgnumber}{int(\pgfplotspointmetatransformed)*2+1}%
	\pgfsetstrokecolor{colorC}%
	\pgfpathmoveto{\pgfqpoint{-.70710678\pgfplotmarksize}{-.70710678\pgfplotmarksize}}%
	\pgfpathlineto{\pgfqpoint{.70710678\pgfplotmarksize}{.70710678\pgfplotmarksize}}%
	\pgfpathmoveto{\pgfqpoint{-.70710678\pgfplotmarksize}{.70710678\pgfplotmarksize}}%
	\pgfpathlineto{\pgfqpoint{.70710678\pgfplotmarksize}{-.70710678\pgfplotmarksize}}%
	\node[actions ocg={ocg\ocgnumber}{}{ocg51 ocg101 ocg151 ocg201 ocg251 ocg301 ocg351 ocg401 ocg451 ocg501 ocg601 ocg701 ocg801 ocg901 ocg1001}, draw opacity=0] {\pgfusepathqstroke};%
}%
%
\def\xminMain{9e-4}
\begin{tikzpicture}%
	\begin{axis}
	[
		point meta min = 0, 
		point meta max = 2000, 
		width	= 1.0\textwidth-15.5pt,
		height	= 0.3\textheight,
		xmode	= log,
		xmin	= \xminMain,
		xmax	= 0.02,
		xlabel	= {$1/L$},
		ylabel	= {GS energy per lattice site $E_0/L$},
		legend style	= {font=\scriptsize, at={(1,0)}, anchor=south east, draw = none, fill=none},
		legend columns = 1,
	]
		\addplot
		[
			color	= colorC,
			scatter,
			mark	= xocgC,
			only marks,
			thick,
			point meta={\thisrowno{0}},
			forget plot,
			error bars/.cd, 
			y dir=both,
			y explicit,
		] 
			table
			[
				x expr = 1.0/\thisrowno{0}, 
				y expr = \thisrowno{2}/\thisrowno{0},
				y error expr = \thisrowno{3}/\thisrowno{0}, 
			]
			{\dstdir/scaling.dat};
%	
		\ifthenelse{\boolean{rebuildData}}%
		{%
			\makeatletter
				\addplot
				[
					no markers, 
					color=blue,
					thick,
					forget plot,
				] %					
					gnuplot 
					[
					raw gnuplot
					] 
					{
						set fit quiet;
						set fit logfile '/dev/null';
						set print "\dstdir/scaling_output.dat" append;
						set fit errorvariables;
						f(x) = a+b*x;
						fit f(x) '\dstdir/scaling.dat' u (1.0/$1):($3/$1):($4/$1) yerrors via a,b;
						print a,a_err,b,b_err;
					};
			\makeatother
		}{}%
%
		\pgfplotstableread[header=false]{\dstdir/scaling_output.dat}{\Data}
		\pgfplotstablegetelem{0}{0}\of\Data 
		\xdef\Ea{\pgfplotsretval}
		\pgfplotstablegetelem{0}{1}\of\Data 
		\xdef\Eaerr{\pgfplotsretval}
		\pgfplotstablegetelem{0}{2}\of\Data 
		\xdef\Eb{\pgfplotsretval}
		\pgfplotstablegetelem{0}{3}\of\Data 
		\xdef\Eberr{\pgfplotsretval}
%			
%			
%			
		\addplot
		[
			mark	= none,
			color	= colorC,
			thick,
			domain	= \xminMain:0.02,
			samples	= 100,
		]
			{linearFct(\Eb, \Ea)};%
%
		\coordinate (epsinf_begin) at (axis cs: 9e-04,\Ea);%
		\coordinate (epsinf_end) at (axis cs: 7.e-03,\Ea);%
		\coordinate (inset_position) at (axis cs:1.15e-3,-2.105);%
		\coordinate (inset_position_var) at (axis cs:3.15e-3,-2.105);%
		\coordinate (inset_position_two) at (axis cs:4.5e-3,-2.105);%
	\end{axis}%
%	
	\draw[thick, densely dotted, draw = colorC] (epsinf_begin) -- (epsinf_end) node[right, font=\scriptsize, fill=white, inner sep = 1pt, xshift=3pt] {$\varepsilon_\infty=\pgfmathprintnumber[std,precision=8,zerofill]{\Ea} \pm \pgfmathprintnumber[sci,precision=0]{\Eaerr}$};%
%	
	\begin{axis}
	[
		at	= {(inset_position)},
		anchor	= north west,
		width	= 0.35\textwidth,
		height	= 0.18\textheight,
		title	= {CPU time},
		xlabel	= {$L$},
		ylabel	= {$t$ [h]},
		title style	= {font=\scriptsize,yshift=-5pt},
		ticklabel style	= {font=\scriptsize},
		xlabel style	= {font=\scriptsize,yshift=5pt},
		ylabel style	= {font=\scriptsize,yshift=-7.5pt},
	]
		\addplot
		[
			color	= colorA,
			mark	= x,
			thick,
			restrict x to domain = 0:501,
		]
			table
			[
				x expr	= \thisrowno{0},
				y expr	= \thisrowno{7}/3600,
			]
			{\dataroot/../finite_size_scaling/t_\t_w_\w_g_\g.symmps.\dw.\blas};
	\end{axis}
		
	\foreach \L in \Ls
	{
		\def\d{1em04}
		\pgfmathsetmacro{\N}{int(\L/2)}
%
		\ifthenelse{\boolean{rebuildData}}%
		{%
			\IfFileExists{\datadir/../gs_energies.dat}%
			{
				\immediate\write18{rm -f  \datadir/../.NoValidResultsDetected.tmp}%
				\immediate\write18%
				{if [ \string$(cat \datadir/../gs_energies.dat | wc -l) = 1 ]; then touch  \datadir/../.NoValidResultsDetected.tmp; fi}%
				\IfFileExists{\datadir/../gs_fit.dat}%
				{
					\immediate\write18%
					{if [ \string$(cat \datadir/../gs_fit.dat | wc -l) = 0 ]; then touch  \datadir/../.NoValidResultsDetected.tmp; fi}%
					\immediate\write18%
					{if [ \string$(grep -v "NaN" \datadir/../gs_fit.dat | wc -l) = 0 ]; then touch  \datadir/../.NoValidResultsDetected.tmp; fi}%
					\immediate\write18%
					{if [ \string$(grep -v "inf" \datadir/../gs_fit.dat | wc -l) = 0 ]; then touch  \datadir/../.NoValidResultsDetected.tmp; fi}%
				}{}%
				
			}%
			{
				\immediate\write18{touch  \datadir/../.NoValidResultsDetected.tmp}%	
			}%
		}{}
		%
		\IfFileExists{\datadir/../.NoValidResultsDetected.tmp}{}%
		{
			\IfFileExists{\datadir/../gs_energies.dat}%
			{
				\pgfplotstableread[header=false]{\datadir/../gs_fit.dat}{\DataUZero}%
				\pgfplotstablegetelem{0}{2}\of\DataUZero%
				\pgfmathsetmacro{\Ea}{\pgfplotsretval}%
				\pgfplotstablegetelem{0}{3}\of\DataUZero% 
				\edef\Eaerr{\pgfplotsretval}%
				\pgfplotstablegetelem{0}{4}\of\DataUZero%
				\pgfmathsetmacro{\Eb}{\pgfplotsretval}%
		%							
				\pgfmathparse{\eval{\Ea/\L}}%
				\edef\E{\pgfmathresult}%
				\pgfmathparse{\eval{\Eaerr}}%
				\edef\Eerr{\pgfmathresult}%
				\begin{axis}
				[
				    y tick label style={
						/pgf/number format/.cd,
						fixed,
						fixed zerofill,
						precision=3,
						/tikz/.cd
					},
					name = ocgplot,
					ocg = {name=ocg\L, ref=ocg\L, status=invisible},
					inner sep=1pt,
					at	=	 {(inset_position_two)},
					anchor	= north west,
					width	=	0.49\textwidth,
					height	=	0.14\textheight,
					xmode	=	log,
					axis background/.style={fill=white, fill opacity=0.9},
					xlabel	=	{\tiny Discarded weight},
					ylabel	=	{\tiny $\nicefrac{E_0}{L}$},
					title	=	{\tiny $L=\L$, $E_0/L=\pgfmathprintnumber[std,precision=4]{\E} \pm \pgfmathprintnumber[sci,precision=1]{\Eerr}$},
					title style={yshift=-0.35em,xshift=-1em,fill=white, name=title},
					every tick label/.append style={font=\tiny,fill=white, fill opacity=0.9},
					xlabel style={name=xlabel,fill=white, fill opacity=0.9},
				]
					\addplot
					[
						color=blue,
						only marks,
						mark=x,
						forget plot,
						unbounded coords=jump,
						error bars/.cd, 
						y dir=both,
						y explicit,
					] 
						table
						[
							x expr = \thisrowno{3},
							y expr = \eval{(\thisrowno{1})/(\L)},
							y error expr = \eval{2.0*sqrt(\thisrowno{3}/\L)}, 
						]
						{\datadir/../gs_energies.dat};
													
					\addplot
					[
						domain	=	\xmin:\xmax,
						color=blue,
						dashed,
					]
						{linearFct(\Eb, \Ea)/\L};
				\end{axis}
			}{}
		}
	}
	\node[actions ocg={}{}{ocg51 ocg101 ocg151 ocg201 ocg251 ocg301 ocg351 ocg401 ocg451 ocg501 ocg601 ocg701 ocg801 ocg901 ocg1001},fit = (title) (xlabel), inner sep = 0,yshift=-0.0625\textheight, inner xsep=2em, xshift=-0.0625\textwidth] {};
\end{tikzpicture}%
